Can We Trust the Performance Evaluation of Uncertainty Estimation Methods in Text Summarization?

Text summarization, a key natural language generation (NLG) task, is vital in various domains. However, the high cost of inaccurate summaries in risk-critical applications, particularly those involving human-in-the-loop decision-making, raises concerns about the reliability of uncertainty estimation on text summarization (UE-TS) evaluation methods. This concern stems from the dependency of uncertainty model metrics on diverse and potentially conflicting NLG metrics. To address this issue, we introduce a comprehensive UE-TS benchmark incorporating 31 NLG metrics across four dimensions. The benchmark evaluates the uncertainty estimation capabilities of two large language models and one pre-trained language model on three datasets, with human-annotation analysis incorporated where applicable. We also assess the performance of 14 common uncertainty estimation methods within this benchmark. Our findings emphasize the importance of considering multiple uncorrelated NLG metrics and diverse uncertainty estimation methods to ensure reliable and efficient evaluation of UE-TS techniques. Our code and data are available https://github.com/he159ok/Benchmark-of-Uncertainty-Estimation-Methods-in-Text-Summarization.

==> img/1-aeslc-kendall.tex <==
% use spearman correlation figures
\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/aeslc_bart_col_UE_ht_kendall.pdf}
\caption{Diagram of Kendall-Tau correlation between uncertainty estimation methods on AESLC dataset. The generated summaries are from BART.}
\label{fig:ken_ue_aes_bart}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/aeslc_bart_row_NLG_ht_kendall.pdf}
\caption{Diagram of Kendall-Tau correlation between NLG metrics on AESLC dataset. The generated summaries are from BART.}
\label{fig:ken_nlg_aes_bart}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/aeslc_gpt35_col_UE_ht_kendall.pdf}
\caption{Diagram of Kendall-Tau correlation between uncertainty estimation methods on AESLC dataset. The generated summaries are from GPT-3.5.}
\label{fig:ken_ue_aes_gpt35}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/aeslc_gpt35_row_NLG_ht_kendall.pdf}
\caption{Diagram of Kendall-Tau correlation between NLG metrics on AESLC dataset. The generated summaries are from GPT-3.5.}
\label{fig:ken_nlg_aes_gpt35}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/aeslc_llama_col_UE_ht_kendall.pdf}
\caption{Diagram of Kendall-Tau correlation between uncertainty estimation methods on AESLC dataset. The generated summaries are from Llama 2.}
\label{fig:ken_ue_aes_llama}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/aeslc_llama_row_NLG_ht_kendall.pdf}
\caption{Diagram of Kendall-Tau correlation between NLG metrics on AESLC dataset. The generated summaries are from Llama 2.}
\label{fig:ken_nlg_aes_llama}
\end{figure*}

==> img/2-xsum-kendall.tex <==
% use spearman correlation figures
\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/xsum_bart_col_UE_ht_kendall.pdf}
\caption{Diagram of Kendall-Tau correlation between uncertainty estimation methods on XSUM dataset. The generated summaries are from BART.}
\label{fig:ken_ue_xsum_bart}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/xsum_bart_row_NLG_ht_kendall.pdf}
\caption{Diagram of Kendall-Tau correlation between NLG metrics on XSUM dataset. The generated summaries are from BART.}
\label{fig:ken_nlg_xsum_bart}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/xsum_gpt35_col_UE_ht_kendall.pdf}
\caption{Diagram of Kendall-Tau correlation between uncertainty estimation methods on XSUM dataset. The generated summaries are from GPT-3.5.}
\label{fig:ken_ue_xsum_gpt35}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/xsum_gpt35_row_NLG_ht_kendall.pdf}
\caption{Diagram of Kendall-Tau correlation between NLG metrics on XSUM dataset. The generated summaries are from GPT-3.5.}
\label{fig:ken_nlg_xsum_gpt35}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/xsum_llama_col_UE_ht_kendall.pdf}
\caption{Diagram of Kendall-Tau correlation between uncertainty estimation methods on XSUM dataset. The generated summaries are from Llama 2.}
\label{fig:ken_ue_xsum_llama}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/xsum_llama_row_NLG_ht_kendall.pdf}
\caption{Diagram of Kendall-Tau correlation between NLG metrics on XSUM dataset. The generated summaries are from Llama 2.}
\label{fig:ken_nlg_xsum_llama}
\end{figure*}

==> img/3-aeslc-spearman.tex <==
% use spearman correlation figures

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/partial35/aeslc_bart_row_NLG_ht_spearman.pdf}
\caption{Diagram of Spearman correlation between NLG metrics on AESLC dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_aes_bart}.  The generated summaries are from BART. For the GPT-3.5-based NLG metrics, we only conduct wo-GPT-3.5 on the BART generation model setting.}
\label{fig:spear_nlg_aes_bart}
\end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/partial35/aeslc_gpt35_row_NLG_ht_spearman_partial35.pdf}
\caption{Diagram of Spearman correlation between NLG metrics on AESLC dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_aes_gpt35}. The generated summaries are from GPT-3.5. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_aes_gpt35}
\end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/partial35/aeslc_llama_row_NLG_ht_spearman_partial35.pdf}
\caption{Diagram of Spearman correlation between NLG metrics on AESLC dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_aes_llama}. The generated summaries are from Llama 2. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_aes_llama}
\end{figure*}


\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/partial35/aeslc_bart_col_UE_ht_spearman.pdf}
\caption{Diagram of Spearman correlation between uncertainty estimation methods on AESLC dataset from the view of NLG metrics used in Fig.~\ref{fig:spear_nlg_aes_bart}. The generated summaries are from BART.}
\label{fig:spear_ue_aes_bart}
\end{figure*}


\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/partial35/aeslc_gpt35_col_UE_ht_spearman_partial35.pdf}
\caption{Diagram of Spearman correlation between uncertainty estimation methods on AESLC dataset from the view of NLG metrics used in Fig.~\ref{fig:spear_nlg_aes_gpt35}.  The generated summaries are from GPT-3.5.}
\label{fig:spear_ue_aes_gpt35}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/partial35/aeslc_llama_col_UE_ht_spearman_partial35.pdf}
\caption{Diagram of Spearman correlation between uncertainty estimation methods on AESLC dataset from the view of NLG metrics used in Fig.~\ref{fig:spear_nlg_aes_llama}.  The generated summaries are from Llama 2.}
\label{fig:spear_ue_aes_llama}
\end{figure*}



==> img/4-xsum-spearman.tex <==
% use spearman correlation figures

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/partial35/xsum_bart_row_NLG_ht_spearman.pdf}
\caption{Diagram of Spearman correlation between NLG metrics on XSUM dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_xsum_bart}.  The generated summaries are from BART. For the GPT-3.5-based NLG metrics, we only conduct wo-GPT-3.5 on the BART generation model setting.}
\label{fig:spear_nlg_xsum_bart}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/partial35/xsum_gpt35_row_NLG_ht_spearman_partial35.pdf}
\caption{Diagram of Spearman correlation between NLG metrics on XSUM dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_xsum_gpt35}. The generated summaries are from GPT-3.5. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_xsum_gpt35}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/partial35/xsum_llama_row_NLG_ht_spearman_partial35.pdf}
\caption{Diagram of Spearman correlation between NLG metrics on XSUM dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_xsum_llama}. The generated summaries are from Llama 2. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_xsum_llama}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/partial35/xsum_bart_col_UE_ht_spearman.pdf}
\caption{Diagram of Spearman correlation between uncertainty estimation methods on XSUM dataset from the view of NLG metrics used in Fig.~\ref{fig:spear_nlg_xsum_bart}. The generated summaries are from BART.}
\label{fig:spear_ue_xsum_bart}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/partial35/xsum_gpt35_col_UE_ht_spearman_partial35.pdf}
\caption{Diagram of Spearman correlation between uncertainty estimation methods on XSUM dataset from the view of NLG metrics used in Fig.~\ref{fig:spear_nlg_xsum_gpt35}. The generated summaries are from GPT-3.5.}
\label{fig:spear_ue_xsum_gpt35}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/partial35/xsum_llama_col_UE_ht_spearman_partial35.pdf}
\caption{Diagram of Spearman correlation between uncertainty estimation methods on XSUM dataset from the view of NLG metrics used in Fig.~\ref{fig:spear_nlg_xsum_llama}. The generated summaries are from Llama 2.}
\label{fig:spear_ue_xsum_llama}
\end{figure*}



==> img/5-aeslc-spearman_met_cat.tex <==
% use spearman correlation figures

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/aeslc_bart_row_NLG_ht_spearman_metcat_Relevance.pdf}
\caption{Diagram of Spearman correlation in terms of relevance between NLG metrics on AESLC dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_aes_bart}.  The generated summaries are from BART. For the GPT-3.5-based NLG metrics, we only conduct wo-GPT-3.5 on the BART generation model setting.}
\label{fig:spear_nlg_aes_relevance_bart}
\end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/aeslc_gpt35_row_NLG_ht_spearman_metcat_Relevance.pdf}
\caption{Diagram of Spearman correlation in terms of relevance between NLG metrics on AESLC dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_aes_gpt35}. The generated summaries are from GPT-3.5. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_aes_relevance_gpt35}
\end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/aeslc_llama_row_NLG_ht_spearman_metcat_Relevance.pdf}
\caption{Diagram of Spearman correlation in terms of relevance between NLG metrics on AESLC dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_aes_llama}. The generated summaries are from Llama 2. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_aes_relevance_llama}
\end{figure*}


\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/aeslc_bart_row_NLG_ht_spearman_metcat_Consistency.pdf}
\caption{Diagram of Spearman correlation in terms of consistency between NLG metrics on AESLC dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_aes_bart}.  The generated summaries are from BART. For the GPT-3.5-based NLG metrics, we only conduct wo-GPT-3.5 on the BART generation model setting.}
\label{fig:spear_nlg_aes_consistency_bart}
\end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/aeslc_gpt35_row_NLG_ht_spearman_metcat_Consistency.pdf}
\caption{Diagram of Spearman correlation in terms of consistency between NLG metrics on AESLC dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_aes_gpt35}. The generated summaries are from GPT-3.5. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_aes_consistency_gpt35}
\end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/aeslc_llama_row_NLG_ht_spearman_metcat_Consistency.pdf}
\caption{Diagram of Spearman correlation in terms of consistency between NLG metrics on AESLC dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_aes_llama}. The generated summaries are from Llama 2. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_aes_consistency_llama}
\end{figure*}

% \begin{figure*}[!htbp]
% \centering
% \includegraphics[width=\textwidth]{./img/met_cat/aeslc_bart_row_NLG_ht_spearman_metcat_Coherence.pdf}
% \caption{Diagram of Spearman correlation in terms of coherence between NLG metrics on AESLC dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_aes_bart}.  The generated summaries are from BART. For the GPT-3.5-based NLG metrics, we only conduct wo-GPT-3.5 on the BART generation model setting.}
% \label{fig:spear_nlg_aes_coherence_bart}
% \end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/aeslc_gpt35_row_NLG_ht_spearman_metcat_Coherence.pdf}
\caption{Diagram of Spearman correlation in terms of coherence between NLG metrics on AESLC dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_aes_gpt35}. The generated summaries are from GPT-3.5. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_aes_coherence_gpt35}
\end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/aeslc_llama_row_NLG_ht_spearman_metcat_Coherence.pdf}
\caption{Diagram of Spearman correlation in terms of coherence between NLG metrics on AESLC dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_aes_llama}. The generated summaries are from Llama 2. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_aes_coherence_llama}
\end{figure*}

% \begin{figure*}[!htbp]
% \centering
% \includegraphics[width=\textwidth]{./img/met_cat/aeslc_bart_row_NLG_ht_spearman_metcat_Fluency.pdf}
% \caption{Diagram of Spearman correlation in terms of fluency between NLG metrics on AESLC dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_aes_bart}.  The generated summaries are from BART. For the GPT-3.5-based NLG metrics, we only conduct wo-GPT-3.5 on the BART generation model setting.}
% \label{fig:spear_nlg_aes_fluency_bart}
% \end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/aeslc_gpt35_row_NLG_ht_spearman_metcat_Fluency.pdf}
\caption{Diagram of Spearman correlation in terms of fluency between NLG metrics on AESLC dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_aes_gpt35}. The generated summaries are from GPT-3.5. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_aes_fluency_gpt35}
\end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/aeslc_llama_row_NLG_ht_spearman_metcat_Fluency.pdf}
\caption{Diagram of Spearman correlation in terms of fluency between NLG metrics on AESLC dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_aes_llama}. The generated summaries are from Llama 2. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_aes_fluency_llama}
\end{figure*}

% \begin{figure*}[!htbp]
% \centering
% \includegraphics[width=\textwidth]{./img/met_cat/aeslc_bart_row_NLG_ht_spearman_metcat_Overall.pdf}
% \caption{Diagram of Spearman correlation in terms of overall between NLG metrics on AESLC dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_aes_bart}.  The generated summaries are from BART. For the GPT-3.5-based NLG metrics, we only conduct wo-GPT-3.5 on the BART generation model setting.}
% \label{fig:spear_nlg_aes_overall_bart}
% \end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/aeslc_gpt35_row_NLG_ht_spearman_metcat_Overall.pdf}
\caption{Diagram of Spearman correlation in terms of overall between NLG metrics on AESLC dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_aes_gpt35}. The generated summaries are from GPT-3.5. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_aes_overall_gpt35}
\end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/aeslc_llama_row_NLG_ht_spearman_metcat_Overall.pdf}
\caption{Diagram of Spearman correlation in terms of overall between NLG metrics on AESLC dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_aes_llama}. The generated summaries are from Llama 2. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_aes_overall_llama}
\end{figure*}

==> img/6-xsum-spearman_met_cat.tex <==
% use spearman correlation figures

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/xsum_bart_row_NLG_ht_spearman_metcat_Relevance.pdf}
\caption{Diagram of Spearman correlation in terms of relevance between NLG metrics on XSUM dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_xsum_bart}.  The generated summaries are from BART. For the GPT-3.5-based NLG metrics, we only conduct wo-GPT-3.5 on the BART generation model setting.}
\label{fig:spear_nlg_xsum_relevance_bart}
\end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/xsum_gpt35_row_NLG_ht_spearman_metcat_Relevance.pdf}
\caption{Diagram of Spearman correlation in terms of relevance between NLG metrics on XSUM dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_xsum_gpt35}. The generated summaries are from GPT-3.5. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_xsum_relevance_gpt35}
\end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/xsum_llama_row_NLG_ht_spearman_metcat_Relevance.pdf}
\caption{Diagram of Spearman correlation in terms of relevance between NLG metrics on XSUM dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_xsum_llama}. The generated summaries are from Llama 2. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_xsum_relevance_llama}
\end{figure*}


\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/xsum_bart_row_NLG_ht_spearman_metcat_Consistency.pdf}
\caption{Diagram of Spearman correlation in terms of consistency between NLG metrics on XSUM dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_xsum_bart}.  The generated summaries are from BART. For the GPT-3.5-based NLG metrics, we only conduct wo-GPT-3.5 on the BART generation model setting.}
\label{fig:spear_nlg_xsum_consistency_bart}
\end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/xsum_gpt35_row_NLG_ht_spearman_metcat_Consistency.pdf}
\caption{Diagram of Spearman correlation in terms of consistency between NLG metrics on XSUM dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_xsum_gpt35}. The generated summaries are from GPT-3.5. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_xsum_consistency_gpt35}
\end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/xsum_llama_row_NLG_ht_spearman_metcat_Consistency.pdf}
\caption{Diagram of Spearman correlation in terms of consistency between NLG metrics on XSUM dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_xsum_llama}. The generated summaries are from Llama 2. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_xsum_consistency_llama}
\end{figure*}

% \begin{figure*}[!htbp]
% \centering
% \includegraphics[width=\textwidth]{./img/met_cat/xsum_bart_row_NLG_ht_spearman_metcat_Coherence.pdf}
% \caption{Diagram of Spearman correlation in terms of coherence between NLG metrics on XSUM dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_xsum_bart}.  The generated summaries are from BART. For the GPT-3.5-based NLG metrics, we only conduct wo-GPT-3.5 on the BART generation model setting.}
% \label{fig:spear_nlg_xsum_coherence_bart}
% \end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/xsum_gpt35_row_NLG_ht_spearman_metcat_Coherence.pdf}
\caption{Diagram of Spearman correlation in terms of coherence between NLG metrics on XSUM dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_xsum_gpt35}. The generated summaries are from GPT-3.5. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_xsum_coherence_gpt35}
\end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/xsum_llama_row_NLG_ht_spearman_metcat_Coherence.pdf}
\caption{Diagram of Spearman correlation in terms of coherence between NLG metrics on XSUM dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_xsum_llama}. The generated summaries are from Llama 2. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_xsum_coherence_llama}
\end{figure*}

% \begin{figure*}[!htbp]
% \centering
% \includegraphics[width=\textwidth]{./img/met_cat/xsum_bart_row_NLG_ht_spearman_metcat_Fluency.pdf}
% \caption{Diagram of Spearman correlation in terms of fluency between NLG metrics on XSUM dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_xsum_bart}.  The generated summaries are from BART. For the GPT-3.5-based NLG metrics, we only conduct wo-GPT-3.5 on the BART generation model setting.}
% \label{fig:spear_nlg_xsum_fluency_bart}
% \end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/xsum_gpt35_row_NLG_ht_spearman_metcat_Fluency.pdf}
\caption{Diagram of Spearman correlation in terms of fluency between NLG metrics on XSUM dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_xsum_gpt35}. The generated summaries are from GPT-3.5. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_xsum_fluency_gpt35}
\end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/xsum_llama_row_NLG_ht_spearman_metcat_Fluency.pdf}
\caption{Diagram of Spearman correlation in terms of fluency between NLG metrics on XSUM dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_xsum_llama}. The generated summaries are from Llama 2. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_xsum_fluency_llama}
\end{figure*}

% \begin{figure*}[!htbp]
% \centering
% \includegraphics[width=\textwidth]{./img/met_cat/xsum_bart_row_NLG_ht_spearman_metcat_Overall.pdf}
% \caption{Diagram of Spearman correlation in terms of overall between NLG metrics on XSUM dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_xsum_bart}.  The generated summaries are from BART. For the GPT-3.5-based NLG metrics, we only conduct wo-GPT-3.5 on the BART generation model setting.}
% \label{fig:spear_nlg_xsum_overall_bart}
% \end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/xsum_gpt35_row_NLG_ht_spearman_metcat_Overall.pdf}
\caption{Diagram of Spearman correlation in terms of overall between NLG metrics on XSUM dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_xsum_gpt35}. The generated summaries are from GPT-3.5. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_xsum_overall_gpt35}
\end{figure*}



\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/met_cat/xsum_llama_row_NLG_ht_spearman_metcat_Overall.pdf}
\caption{Diagram of Spearman correlation in terms of overall between NLG metrics on XSUM dataset from the view of uncertainty estimation methods used in Fig.~\ref{fig:spear_ue_xsum_llama}. The generated summaries are from Llama 2. For the GPT-3.5-based NLG metrics, we only draw wi-ingt-GPT-3.5 results to save space.}
\label{fig:spear_nlg_xsum_overall_llama}
\end{figure*}

==> img/7-tofu-spearman.tex <==
% use spearman correlation figures

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/tofu_partial35/tofu_gpt35_col_UE_ht_spearman_partial35_unc_nlg.pdf}
\caption{Diagram of Spearman correlation between uncertainty estimation on TofuEval dataset from the view of NLG metrics.  The generated summaries are from GPT-3.5. }
\label{fig:spear_ue_nlg_tofu_gpt35}
\end{figure*}



% use spearman correlation figures

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/tofu_partial35/tofu_gpt35_col_UE_ht_spearman_partial35_unc_hum.pdf}
\caption{Diagram of Spearman correlation between uncertainty estimation on TofuEval dataset from the view of human annotation.  The generated summaries are from GPT-3.5. }
\label{fig:spear_ue_hum_tofu_gpt35}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\textwidth]{./img/tofu_partial35/tofu_gpt35_col_UE_ht_spearman_partial35_nlg_hum.pdf}
\caption{Diagram of Spearman correlation between NLG metrics on TofuEval dataset from the view of human annotation.  The generated summaries are from GPT-3.5. }
\label{fig:spear_nlg_hum_tofu_gpt35}
\end{figure*}
